A Simple and Practical Concurrent Non-blocking Unbounded Graph with Reachability Queries

Graph algorithms applied in many applications, including social networks, communication networks, VLSI design, graphics, and several others, require dynamic modifications -- addition and removal of vertices and/or edges -- in the graph. This paper presents a novel concurrent non-blocking algorithm to implement a dynamic unbounded directed graph in a shared-memory machine. The addition and removal operations of vertices and edges are lock-free. For a finite sized graph, the lookup operations are wait-free. Most significant component of the presented algorithm is the reachability query in a concurrent graph. The reachability queries in our algorithm are obstruction-free and thus impose minimal additional synchronization cost over other operations. We prove that each of the data structure operations are linearizable. We extensively evaluate a sample C/C++ implementation of the algorithm through a number of micro-benchmarks. The experimental results show that the proposed algorithm scales well with the number of threads and on an average provides 5 to 7x performance improvement over a concurrent graph implementation using coarse-grained locking.

==> code/code2.tex <==
\begin{figure*}[!htp]
\captionsetup{font=footnotesize}
	\begin{subfigure}{.33\textwidth}	
\begin{algorithmic}[1]
	%\algrestore{locv}
	\algrestore{locvplus}
	\small
		\Procedure{$\convplus$ ($k$, $l$)}{}\label{convpstart}
		\If{($k < l$)}
		\State {$\langle pv1, cv1\rangle$ $\gets$ $\locvplus$($\vh$, $k$)} \label{lin:locvplus-k}
		\If{($cv1.k$ $\neq$ $k$)}
	     \State{return $\langle \nul, \nul, \fal \rangle$;}
		\EndIf
		\State {$\langle pv2, cv2\rangle$ $\gets$ $\locvplus$($cv1$, $l$)} \label{lin:locvplus-l}
		\If{($cv2.k$ $\neq$ $l$)}
	     \State{return $\langle \nul, \nul, \fal \rangle$;}
		\EndIf
		\Else
		\State {$\langle pv2, cv2\rangle$ $\gets$ $\locvplus$($\vh$, $l$)}
		\If{($cv2.k$ $\neq$ $l$)}
	     \State{return $\langle \nul, \nul, \fal \rangle$;}
		\EndIf
		\State {$\langle pv1, cv1\rangle$ $\gets$ $\locvplus$($cv2$, $k$)}
		\If{($cv1.k$ $\neq$ $k$)}
	     \State{return $\langle \nul, \nul, \fal \rangle$ ;} 
		\EndIf
		\EndIf
		\State {returns $\langle cv1, cv2, \tru \rangle$;} 
        \EndProcedure\label{convpend}
		\algstore{convplus}
\end{algorithmic}
	%\caption{}\label{conv}
	\end{subfigure}
    \begin{subfigure}{.33\textwidth}
	\begin{algorithmic}[1]
	\algrestore{convplus}
\renewcommand{\algorithmicprocedure}{\textbf{Operation}}	
	\small
		\Procedure{ $\adde$($k$, $l$)}{}\label{addestart}
		\State {$\langle$ u, v, st $\rangle$ $\gets$ $\convplus$($k, l);$}  \label{lin:adde-convplus}
		 \If{(st = \fal)}
		%\State{$flag \gets false$;}
        \State {return ``\vntp`` ; }
        \EndIf
        \While{(\tru)}
	 \If{(\isMarked($u$) $\bigvee$  \isMarked($v$))}	\label{lin:adde-check-uv}
        \State return ``\vntp``; 
        \EndIf
		\State{$\langle pe, ce \rangle$ $\gets$ \loceplus ($u.\enext$, $l$);} \label{lin:adde-loceplus}
		\If{($ce.l$ $=$ $l$)}
		\State return ``\ep``; 
		\EndIf
		
       
        \State{$ne$ $\gets$ \createe($l$);}
		\State{$ne.\enext$ $\gets$ $ce$}
		\State{$ne.\pointv$ $\gets$ $v$}
		\If{(CAS($pe.\enext$, $ce, ne   $))}\label{lin:cas-adde}
         \State{u.\ecount.\fadd(1);}\label{faa:ade}
		\State return ``\eadd``;
		\EndIf
		
		\EndWhile
        \EndProcedure\label{addeend}
		\algstore{adde}
\end{algorithmic}
		%\caption{}\label{remv}
	\end{subfigure}
	 \begin{subfigure}{.33\textwidth}
	\begin{algorithmic}[1]
	\algrestore{adde}
	\small
\renewcommand{\algorithmicprocedure}{\textbf{Operation}}	
		\Procedure{ $\reme$($k$, $l$)}{}\label{remestart}
    		\State {$\langle$ u, v, st $\rangle$ $\gets$ $\convplus$($k, l);$}  \label{lin:reme-validate-u}
		 \If {(st = \fal)}
	    \State {return ``\vntp``; }
       \EndIf
       	\While{(\tru)}
       	        \If{(\isMarked($u$) $\bigvee$  \isMarked($v$))}	\label{lin:reme-check-uv}
        \State return ``\vntp``; 
        \EndIf
		\State{$\langle pe, ce \rangle$ $\gets$ \loceplus ($u.\enext$, $l$);} \label{lin:reme-loceplus}
		\If{($ce.l$ $\neq$ $l$)}
		\State return ``\entp``; 
		\EndIf
		
		\State{$cnt$ $\gets$ $ce.\enext$;}
		\If{($\neg$ \isMarked($cnt$))} 
		\If{(CAS($ce.\enext$, $cnt$, \MarkedRef($cnt$)))} \label{lin:cas-reme}
		 \State{u.\ecount.\fadd(1);}\label{increm}
		 \If{(CAS($pe.\enext, ce, cnt$))} \label{lin:cas-reme-phy}%// physical deletion
        \State{ $break$;} 
        \EndIf
        
		\EndIf
		\EndIf
		\EndWhile
		\State return ``\er``; 
	    \EndProcedure\label{remeend}
        \algstore{reme}
\end{algorithmic}
		%\caption{}\label{locvplus}
	\end{subfigure}
	\caption{Pseudo-codes of \convplus, \adde and \reme methods.}\label{fig:e-methods}
\end{figure*}

==> code/getpathcode2.tex <==
\begin{figure*}[!htp]
\captionsetup{font=footnotesize}
	\begin{subfigure}{.45\textwidth}	
\begin{algorithmic}[1]
	\algrestore{comparepath}
	\small
		\Procedure{ $\adde$($k$, $l$)}{}
		\State {$\langle$ u, v, st $\rangle$ $\gets$ $\convplus$($k, l);$}  \label{lin:adde-convplus-g}
		 \If{(st = \fal)}
		%\State{$flag \gets false$;}
        \State {return ''VERTEX NOT PRESENT'' ; }
        \EndIf
        \While{(\tru)}
	\If{(\isMarked($u$) $\bigvee$  \isMarked($v$))}	\label{lin:adde-check-uv-g}
        \State return ''VERTEX NOT PRESENT''; 
        \EndIf
		\State{$\langle pe, ce \rangle$ $\gets$ \loceplus ($u.\enext$, $l$);} \label{lin:adde-loceplus-g}
		\If{($ce.val$ $=$ $l$)}
		\State return ''EDGE EXISTS''; 
		\EndIf
		
        
        \State{$ne$ $\gets$ \createe($l$);}
		\State{$ne.\enext$ $\gets$ $ce$}
		\State{$ne.\pointv$ $\gets$ $v$}
		\If{(CAS($pe.\enext$, $ce, ne   $))}\label{lin:cas-adde-g}
		 \State{u.\ecount.\fadd(1);}
		\State return ''ADDED'';
		\EndIf
		
		\EndWhile
        \EndProcedure
		\algstore{adde}
\end{algorithmic}
		%\caption{}\label{remv}
	\end{subfigure}
	 \begin{subfigure}{.45\textwidth}
	\begin{algorithmic}[1]
	\algrestore{adde}
	\small
		\Procedure{ $\reme$($k$, $l$)}{}
    		\State {$\langle$ u, v, st $\rangle$ $\gets$ $\convplus$($k, l);$}  \label{lin:reme-validate-u-g}
		 \If {(st = \fal)}
	    \State {return ''VERTEX NOT PRESENT''; }
       \EndIf
       	\While{(\tru)}
       	\If{(\isMarked($u$) $\bigvee$  \isMarked($v$))}	\label{lin:reme-check-uv-g}
        \State return ''VERTEX NOT PRESENT''; 
        \EndIf
		\State{$\langle pe, ce \rangle$ $\gets$ \loceplus ($u.\enext$, $l$);} \label{lin:reme-loceplus-g}
		\If{($ce.val$ $\neq$ $l$)}
		\State return ''EDGE DOES NOT EXISTS''; 
		\EndIf
		
		\State{$cnt$ $\gets$ $ce.\enext$;}
		\If{($\neg$ \isMarked($cnt$))} 
		\If{(CAS($ce.\enext$, $cnt$, \MarkedRef($cnt$)))} \label{lin:cas-reme-g}
		%\State{ $break$;} 
		 \State{u.ecount.\fadd(1);}
		 \If{(CAS($pe.\enext, ce, cnt$))} \label{lin:cas-reme-phy-g}%// physical deletion
		
		\State{ $break$;} 
        \EndIf
        
		\EndIf
		\EndIf
		\EndWhile
		\State return ''REMOVED''; 
	    \EndProcedure
       % \algstore{reme}
\end{algorithmic}
		%\caption{}\label{locvplus}
	\end{subfigure}
	\caption{Edge methods for \getpath.}\label{sec:e-methods}
\end{figure*}

==> graphDS.tex <==
%%\vspace{-3mm}
\section{The Graph Data-Structure}%Construction of Concurrent

%In this section, we describe the construction of our concurrent graph \ds. 
We represent a graph by its adjacency list, which we design as a composition (linked-list) of linked-lists. We call the composite linked-list the \textit{vList}. Each node in the vList corresponds to a $v(k) \in V$ and roots a linked-list called an \textit{eList}. Nodes in an eList rooted at correspond to $v(j) \in V$ such that which it has outgoing edges. For clarity, we term  to denote the the linked-lists representing adjacency of \vcs, whereas, \textit{vertex-list} denotes the linked-list of \vcs

In each list, nodes are sorted in order of their keys, providing a convenient way to detect when an item is absent. 

The operations in the graph utilize the linked-list operations -- \add, \rem, \con -- and impose their own semantics on top of them. This enables us to transfer concurrency and liveness, essentially lock-freedom, of the linked-list operations to the graph operations. %We use lock-free linked-list by Harris \cite{Harrisdisc01} to design the lock-free graph.  %To ensure that, we employ concurrent linked-lists as the underlying linked-list in the design.
A typical our graph data structure has two types of nodes \enode and \vnode depicts in the \figref{struct-evnode}. The \enode design contains two pointers in addition to an immutable key field {\tt val}: see class \enode. The \pointv and \enext fields are the atomic references to the corresponding vertex  node in the \vlist and the next edge node in the \elist of a vertex respectively. Similarly, the \vnode also has two pointers and an immutable key  field {\tt val}: see class \vnode. The \vnext and \enext fields are the atomic references to the next vertex node in the \vlist and the next edge head sentinel in the \elist (e.g. adjacency list) of that vertex respectively.  The atomic reference used both in the \enext of \enode and \vnext of \vnode class is the similar to \lf list \cite{Harrisdisc01}, which encapsulates both a reference and a boolean mark field. These fields can be atomically updated, either together or individually. We assume that all the \vcs have a unique identification key (captured by \texttt{val} field) as shown in the \figref{struct-evnode}. We also assume that a vertex once deleted is inserted again with the same key but with different memory address. Further, in the context of a particular application, the node structure can be easily modified to carry useful data (like weights etc). 

The \figref{struct-evnode} depicts the structure of the \enode and \vnode \ignore{list-based set }class. The \vnode creates two sentinel nodes for \vlist, called \vh and \vt. A \vlist can be uniquely identified using its head node. Each vertex of the \vlist also creates two sentinel nodes for its \elist, called \eh and \et. The \eh's \pointv of each vertex points to its vertex and the \et's \pointv pointed to \vt.  An object of the Graph class exports the methods - \addv{(x)}, \remv{(x)}, \conv{(x)}, \adde{(x)}, \reme{(x)} and \cone{(x),}. Each of these methods can be implemented using well-known synchronization techniques of the concurrent set implementation - \emph{fine-grained \cite[Chap. 9]{MauriceNir}, optimistic \cite[Chap. 9]{MauriceNir}, lazy \cite{Heller-PPL2007}} or \emph{lock-free}\cite{Harrisdisc01}. Although in this paper, we mainly focus on the \emph{lock-free} implementation. 
 
